SIPSA-Net: Shift-Invariant Pan Sharpening with Moving Object Alignment for Satellite Imagery

Pan-sharpening is a process of merging a high-resolution (HR) panchromatic (PAN) image and its corresponding low-resolution (LR) multi-spectral (MS) image to create an HR-MS and pan-sharpened image. However, due to the different sensors' locations, characteristics and acquisition time, PAN and MS image pairs often tend to have various amounts of misalignment. Conventional deep-learning-based methods that were trained with such misaligned PAN-MS image pairs suffer from diverse artifacts such as double-edge and blur artifacts in the resultant PAN-sharpened images. In this paper, we propose a novel framework called shift-invariant pan-sharpening with moving object alignment (SIPSA-Net) which is the first method to take into account such large misalignment of moving object regions for PAN sharpening. The SISPA-Net has a feature alignment module (FAM) that can adjust one feature to be aligned to another feature, even between the two different PAN and MS domains. For better alignment in pan-sharpened images, a shift-invariant spectral loss is newly designed, which ignores the inherent misalignment in the original MS input, thereby having the same effect as optimizing the spectral loss with a well-aligned MS image. Extensive experimental results show that our SIPSA-Net can generate pan-sharpened images with remarkable improvements in terms of visual quality and alignment, compared to the state-of-the-art methods.

==> qualitative_table/for_itrc.tex <==
\def\arraystretch{1.2}
\begin{tabular}{l|ccc|cc|ccc}
\hline
 & \multicolumn{3}{c|}{Lower scale (with aligned MS)} & \multicolumn{2}{c|}{Full-scale (with aligned MS)} & \multicolumn{3}{c}{Lower-scale (with misaligned MS)}\\ \cline{2-9}

 & $SCC$ $\uparrow$ & $ERGAS$ $\downarrow$ & $PSNR$ $\uparrow$ & $SCC_{F}$ $\uparrow$ & $QNR$ $\uparrow$  & $SCC$ $\uparrow$ & $ERGAS$ $\downarrow$ & $PSNR$ $\uparrow$\\
\hline
Brovey \cite{brovey} & 0.932 &6.129&27.655 & 0.952 & 0.780  & 0.836 & 7.19  & 26.098 \\ 
Affinity \cite{affinity} & 0.873 & 3.453 & 33.264 & 0.747 & 0.677   & 0.791 & 3.993  & 32.207\\
GF \cite{guided} & 0.886 & 3.394 & 33.376 & 0.778 & 0.680   & 0.801 & 4.005 &  32.175\\
IHS \cite{ihs} & 0.928 & 2.763 & 35.3909 & 0.958 & 0.852 & 0.836 & 3.877 & 32.676  \\
PCA \cite{pca} & 0.908 & 4.575 & 31.187  & 0.899 & 0.743  & 0.817 & 5.06  & 30.41\\
P+XS \cite{pxs}& 0.898 & 3.402 & 32.553 & 0.858 & 0.851  & 0.775 & 4.459 & 30.365\\
Variational \cite{variational} & 0.839 & 2.931 & 35.379 & 0.665 & 0.754  & 0.781 & \underline{3.638} & \underline{33.415} \\
\hline
PanNet \cite{pannet} & 0.877 & 3.315 & 34.113 & 0.811 & 0.806  & 0.802 & 4.047 & 32.374\\
PanNet-S3 \cite{s3} & 0.933 & 2.724 & 35.454 & 0.954 & 0.844  & 0.838 & 3.816 & 32.769 \\
DSen2 \cite{dsen2} & 0.82  & 3.763 & 32.939 & 0.837 & \underline{0.852}  & 0.82  & 3.763 & 32.939 \\
DSen2-S3 \cite{s3} & 0.829 & 2.931 & 35.057  & {0.959} & 0.808  & \textbf{0.844} & 5.33  & 29.39\\
\hline
SIPSA-Net & \textbf{0.940} & \textbf{2.351} & \textbf{36.905} & \textbf{0.964}&  \textbf{0.858}  & \textbf{0.844} & \textbf{3.505} & \textbf{33.662}\\	

\hline
\end{tabular}


==> qualitative_table/qnr_jqm.tex <==
\def\arraystretch{1.2}
\begin{tabular}{l|cc|cc}
\hline
 & \multicolumn{2}{c|}{with aligned MS} & \multicolumn{2}{c}{with misaligned MS}\\ \cline{2-5}

 & $QNR$ $\uparrow$ & $JQM$ $\uparrow$ & $QNR$ $\uparrow$ & $JQM$ $\uparrow$ \\\hline
P+XS \cite{pxs}& 0.860 & 0.921 & 0.869 & 0.919 \\
Variational \cite{variational} & 0.894 & 0.913 & 0.902 & 0.926\\
PanNet \cite{pannet} & 0.836 & 0.883 & 0.844 & 0.891 \\
PanNet-S3 \cite{s3} & \underline{0.947} & 0.947 & \underline{0.939} & 0.941 \\
DSen2 \cite{dsen2} & 0.848  & 0.894 & 0.856 & 0.900  \\
DSen2-S3 \cite{s3} & 0.898 & \underline{0.956} & 0.889  & 0.947 \\
\hline
SIPSA-Net (full) & 0.899 & \textbf{0.962} & 0.890  & \textbf{0.955}\\
SIPSA-Net (w/o SiS) & \textbf{0.954} & 0.951 & \textbf{0.947} & \textbf{0.955}\\	

\hline
\end{tabular}


==> qualitative_table/qnr_jqm_withS3.tex <==
\def\arraystretch{1.2}
\begin{tabular}{l|cc|cc}
\hline
 & \multicolumn{2}{c|}{with aligned MS} & \multicolumn{2}{c}{with misaligned MS}\\ \cline{2-5}

 & $QNR$ $\uparrow$ & $JQM$ $\uparrow$ & $QNR$ $\uparrow$ & $JQM$ $\uparrow$ \\\hline
P+XS \cite{pxs}& 0.860 & 0.921 & 0.869 & 0.919 \\
Variational \cite{variational} & 0.894 & 0.913 & 0.902 & 0.926\\
PanNet \cite{pannet} & 0.836 & 0.883 & 0.844 & 0.891 \\
PanNet-S3 \cite{s3} \underline{& 0.947} & 0.947 & 0.939 & 0.941 \\
DSen2 \cite{dsen2} & 0.848  & 0.894 & 0.856 & 0.900  \\
DSen2-S3 \cite{s3} & 0.898 & \underline{0.956} & 0.889  & 0.947 \\
\hline
SIPSA-Net (full) & 0.899 & \textbf{0.962} & 0.890  & \textbf{0.955}\\
SIPSA-Net (w/o SiS) & \textbf{0.954} & 0.951 & \textbf{0.947} & \textbf{0.955}\\	

\hline
\end{tabular}


==> qualitative_table/qualititave.tex <==
\def\arraystretch{1.2}
\begin{tabular}{l|cc|ccc|ccc}
\hline
 & \multicolumn{2}{c|}{Lower-scale (with misaligned MS)} & \multicolumn{3}{c|}{Full-scale} & \multicolumn{3}{c}{lower scale (with aligned MS)}\\ \cline{2-9}

 & $SCC$ $\uparrow$ & $ERGAS$ $\downarrow$ & $SCC_{F}$ $\uparrow$ & $QNR$ $\uparrow$ & $JQM$ $\uparrow$ & $SCC$ $\uparrow$ & $ERGAS$ $\downarrow$ & $PSNR$ $\uparrow$\\
\hline
Brovey \cite{brovey} & 0.836 & 7.19  & 0.952 & 0.780 & 0.884 & 0.932 &6.129&27.655 \\ 
Affinity \cite{affinity} & 0.791 & 3.993  & 0.747 & 0.677 & 0.759 & 0.873 & 3.453 & 33.264\\
GF \cite{guided} & 0.801 & 4.005 & 0.778 & 0.680 & 0.761 & 0.886 & 3.394 & 33.376\\
IHS \cite{ihs} & 0.836 & 3.877 & 0.958 & 0.852 & 0.883 & 0.928 & 2.763 & 35.391  \\
PCA \cite{pca} & 0.817 & 5.06   & 0.899 & 0.743 & 0.845 & 0.908 & 4.575 & 31.187\\
P+XS \cite{pxs} & 0.775 & 4.459  & 0.858 & 0.851 & 0.863 & 0.898 & 3.402 & 32.553\\
PNN \cite{pnn} & 0.762 & 5.1109  & 30.612 & 0.697 & 0.649 & 0.752 & 0.694 & 5.694 & 29.594\\
Variational \cite{variational} & 0.781 & \underline{3.638}  & 0.665 & 0.754 & 0.752 & 0.839 & 2.931 & 35.379\\
\hline
PanNet \cite{pannet} & 0.802 & 4.047  & 0.811 & 0.806 & \underline{0.916} & 0.877 & 3.315 & 34.113\\
PanNet-S3 \cite{s3} & 0.838 & 3.816 & 0.954 & 0.844 & 0.827 & 0.933 & 2.724 & 35.454\\
DSen2 \cite{dsen2} & 0.82  & 3.763 & 0.837 & \underline{0.852} & 0.908 & 0.829 & 2.931 & 35.057\\
DSen2-S3 \cite{s3} & \textbf{0.844} & 5.33    & {0.959} & 0.808 & 0.758 & 0.822 & 4.390 & 31.213\\
\hline
SIPSA-Net (full) & \underline{0.842} & 3.683   & \underline{0.962}&  0.798 & \textbf{0.934} & \textbf{0.940} & \underline{2.500} & \underline{36.354}\\	
SIPSA-Net (w/o SiS) & \textbf{0.844} & \textbf{3.505}   & \textbf{0.964}&  \textbf{0.858} & 0.906 & \textbf{0.940} & \textbf{2.351} & \textbf{36.905}\\	

\hline
\end{tabular}

